Convergence and Diversity in the Control Hierarchy

Weir has defined a hierarchy of language classes whose second member ($\mathcal{L}_2$) is generated by tree-adjoining grammars (TAG), linear indexed grammars (LIG), combinatory categorial grammars, and head grammars. The hierarchy is obtained using the mechanism of control, and $\mathcal{L}_2$ is obtained using a context-free grammar (CFG) whose derivations are controlled by another CFG. We adapt Weir's definition of a controllable CFG to give a definition of controllable pushdown automata (PDAs). This yields three new characterizations of $\mathcal{L}_2$ as the class of languages generated by PDAs controlling PDAs, PDAs controlling CFGs, and CFGs controlling PDAs. We show that these four formalisms are not only weakly equivalent but equivalent in a stricter sense that we call d-weak equivalence. Furthermore, using an even stricter notion of equivalence called d-strong equivalence, we make precise the intuition that a CFG controlling a CFG is a TAG, a PDA controlling a PDA is an embedded PDA, and a PDA controlling a CFG is a LIG. The fourth member of this family, a CFG controlling a PDA, does not correspond to any formalism we know of, so we invent one and call it a Pushdown Adjoining Automaton.

==> discarded.tex <==
% \subsection{Terms}

% \begin{defin}
% We define the set of \defn{terms} $\mathcal{T}(\signature)$ on signature $\signature$ as the smallest set such that
% \begin{itemize}
%     \item $f \in \mathcal{T}(\signature)$ if $f$ has arity $0$;
%     \item $f(t_1, \ldots, t_k) \in \mathcal{T}(\signature)$ if $f$ has arity $k$ and $t_1, \ldots, t_k \in \mathcal{T}(\signature)$.
% \end{itemize}
% \end{defin}

% Since a term has a hierarchical structure, it can be seen as a labeled tree with operation symbols from $\signature$. Each node can be assigned a string of natural numbers indicating its position in the tree. Sometimes it will be convenient to treat a term $t$ as a partial function $t \colon \mathbb{N} ^* \rightharpoonup \signature$ with domain $\pos{}(t)$. 

% \begin{defin}
% The \defn{domain} of a tree $t$, denoted by $\pos{}(t)$ is a set satisfying the following properties:
% \begin{itemize}
%     \item $\pos{}(t)$ is non-empty and prefix-closed;
%     \item $\varepsilon \in \pos{}(t)$ is the position of the root node;
%     \item $\forall p \in \pos{}(t)$, if $t(p)$ has arity $k \geq 1$, then $\{j \mid pj \in \pos{}(t) \}= \{1, \ldots, k \}$;
%     \item $\forall p \in \pos{}(t)$, if $t(p)$ has arity $0$, then $\{j \mid pj \in \pos{}(t) \}= \emptyset$.
% \end{itemize}
% \end{defin}

% We denote by $t|_p$ the subtree of $t$ that starts at position $p$ and by $t[u]_p$ the term obtained by replacing the subtree at $p$ in $t$ with a new tree $u$.



% \subsection{Algebras}
% \ryan{This introduction is way to hard. As someone who didn't read the Burris and Sankappanava book, I don't understand what is meant by operation. \response{alexandra} does it read better now? \response{david} perhaps a gentler way to do this would be to remind readers of the definition of semiring first, since many people already know that?}

% The reader may already be familiar with semirings, which consist of a set $\carrierset$, called the carrier set, together with two distinguished elements $\zero$ and $\one$ and two operations $\oplus$ and $\otimes$. It is common to write generic algorithms in terms of semiring operations and instantiate the algorithms by interpreting the semiring operations in various ways. 
% Here, we introduce some basic notions from universal algebra \citep{burris+:2012}, which generalize to any number and type of operations.

% \begin{defin}
% A \defn{signature} $\signature$ is a set of \defn{operation symbols}, each with an associated \defn{arity}.
% \end{defin}

% \begin{defin}
% We define the set of \defn{terms} $\mathcal{T}(\signature)$ on signature $\signature$ as the smallest set such that

% \begin{compactitem}
%     \item $f \in \mathcal{T}(\signature)$ if $f$ has arity $0$;
%     \item $f(t_1, \ldots, t_k) \in \mathcal{T}(\signature)$ if $f$ has arity $k$ and $t_1, \ldots, t_k \in \mathcal{T}(\signature)$.
% \end{compactitem}
% \end{defin}

% For example, the signature of a semiring is $\{\zero, \one, \oplus, \otimes\}$, and an example term is $(\zero \oplus \one) \otimes (\zero \oplus \one)$.\ryan{I would give a more interesting example with a carrier set. It's a bit hard to follow why we want carrier sets and signatures. \response{alexandra} would it be enough to include also that a term in $\carrierset$ is obtained by applying operations in $\signature$ to other terms in $\carrierset$?}

% \begin{defin}
% %For a nonempty set $\carrierset$ and a nonnegative integer $n$ we define $\carrierset^n$ as the set of $n$-tuples from $\carrierset$. 
% A (partial) \defn{$k$-ary operation} on a nonempty set $\carrierset$ is a (partial) function $f \colon \carrierset^k \rightarrow \carrierset$. We call $k$ the \defn{arity} of $f$. If the operation $f$ is $0$-ary, $1$-ary or $2$-ary, we call it \defn{nullary}, \defn{unary} or \defn{binary}, respectively. A nullary operation on $\carrierset$ is just an element of $\carrierset$.
% \end{defin}

% \begin{defin}
% A (partial) \defn{algebra} is a tuple $(\carrierset, \signature, \interp{\mathord\cdot})$ where:
% \begin{compactitem}
% \item $\carrierset$ is a nonempty set, called the \defn{carrier set}.
% \item $\signature$ is a signature.
% \item For each operation symbol $f$ in $\signature$ with arity $k$, $\interp{f}$ is a (partial) $k$-ary operation on $\carrierset$.
% \end{compactitem}
% \end{defin}\ryan{I would make it clearer why we are using semantic braces.}

% For example, in the real semiring, $\carrierset = \mathbb{R}$, $\interp{\zero} = 0$, $\interp{\one} = 1$, $\interp{\oplus}$ is real addition, and $\interp{\otimes}$ is real multiplication.

% \begin{defin} \label{def:isomorphism}
% Let $\algebra = (\carrierset,\signature,\interp{\mathord\cdot}_{\algebra})$ and $\algebra'=(\carrierset',\signature,\interp{\mathord\cdot}_{\algebra'})$ be two algebras with the same signature $\signature$. A bijection $\phi \colon \carrierset \rightarrow \carrierset'$ is an \defn{isomorphism} from $\algebra$ to $\algebra'$ if for all operation symbols $f \in \signature$ of arity $k$ and all $c_1, \ldots, c_k \in \carrierset$ we have 
% \begin{equation*}
%     \phi (\interp{f}_{\algebra}(c_1,\ldots,c_k)) = \interp{f}_{\algebra'} (\phi(c_1),\ldots,\phi(c_k)).
% \end{equation*}
% If there is such a function $\phi$, we call $\algebra$ and $\algebra'$ \defn{isomorphic}. 
% \end{defin}

% From now on, we use several shorthands. When it is clear which interpretation $\interp{\mathord\cdot}$ is meant, we write $\interp{f}$ simply as~$f$.
% When mentioning an algebra $(\carrierset, \{f_1, \ldots, f_n\}, \interp{\mathord\cdot})$ for the first time, we often write it as $(\carrierset, f_1, \ldots, f_n)$. Subsequently, we often write it simply as $\carrierset$.

\subsection{Monoids}
\alexandra{I removed monoids since we weren't using them}
\begin{defin}
A \defn{monoid} is an algebra $(\semiringset, \odot, \id)$, where $\odot$ is an associative binary operation, and $\id$, called the \defn{identity} element, is a nullary operation satisfying $\id \odot a = a \odot \id = a$ for all $a \in \semiringset$. If $a \odot b = b \odot a$ for all $a,b$, we say that the monoid is \defn{commutative}. 
\end{defin}

\begin{defin}
Let $\alphabet$ be a finite alphabet and let $\wtset$ be a monoid of weights with identity $\id$ and multiplication operation $\otimes$.
The monoid of \defn{weighted strings} over $\alphabet$ and $\wtset$, written $\wtkleene{\alphabet}$, is the set of pairs $\{\langle \str, k\rangle \mid \str \in \alphabet^*, k \in \wtset\}$ with identity $\langle \varepsilon, \id\rangle$ and multiplication operation $\langle \str_1, k_1\rangle \langle \str_2, k_2 \rangle = \langle \str_1 \str_2, k_1 \otimes k_2\rangle$.
\end{defin}\ryan{Did we mention how we denote string concatenation? \response{alexandra} I added it at the beginning of the section}

Whenever $\wtset=(\{ \zero, \one \},\wedge,\one)$, we will write $\str$ for a  weighted string $\langle\str,\one\rangle$ and simply call it a string.

% \begin{defin}
% A \defn{semiring} is an algebra $\semiringtuple$
% such that $\left(\semiringset, \oplus, \zero \right)$ is a commutative monoid and $\left(\semiringset, \otimes, \one \right)$ is a monoid. Additionally, $\otimes$ distributes over $\oplus$, that is, $a \otimes (b \oplus c) = a \otimes b \oplus a \otimes c$ and $(a \oplus b) \otimes c = a \otimes c \oplus b \otimes c$, and $\zero$ is absorbing with respect to $\otimes$, that is, $\zero \otimes a = a \otimes \zero = \zero$. 
% % If $\otimes$ is commutative then we say that $\semiring$ is \defn{commutative}.
% \end{defin}


% We use the term \emph{formal system} to refer generically to either grammars or automata.

% \begin{defin} \label{def:formal-system}
% Let $\signature$ be a signature and $\mathbf{M}$ a monoid (usually of strings or weighted strings). A (weighted) \defn{formal system} over $\mathbf{M}$ is a partial algebra of \defn{derivations} $\carrierset$ together with a partial function, called the \defn{yield function}, $\yield \colon \carrierset \rightharpoonup \mathbf{M}$.\footnote{The algebra is partial because operations can only apply to certain subderivations (e.g., transitions can only apply to configurations with matching states). This situation could have been avoided using many-sorted algebras, but partiality seemed to us to be the simpler solution. The reason $\yield$ is a partial function because, in some formalisms, it may not make sense for a partial derivation to yield a string or it may yield a non-contiguous string.}
% \end{defin}
%  The operations of the algebra correspond to rules or transitions of the formal system; they are partial functions because most formalisms have restrictions on when rules or transitions can apply.

% \david{I think it should be straightforward to define what the configurations, transitions, etc., of an X-controlling-Y are in terms of the configurations, transitions, etc., of X and Y. However, it might look weird to a reader who expects that X controlling Y means that X generates the derivation trees of Y.}

% We now define two notions of equivalence that are stricter than weak equivalence. Suppose two grammars generate, say, the language $\{\sym{a}\}$, but one grammar generates it unambiguously (there is exactly one derivation generating $\sym{a}$) and the other generates it ambiguously (there are two or more, or even infinitely many, derivations generating $\sym{a}$). The two grammars are weakly equivalent, but we want a notion of equivalence that distinguishes these two grammars.
% \begin{defin} \label{def:formal-system-equivalence}
% Two formal systems $(\carrierset_1, \yield_1)$ and $(\carrierset_2, \yield_2)$ over the same monoid are \defn{\bijeqJJ} if there is a bijection $\phi \colon \dom{\yield_1} \rightarrow \dom{\yield_2}$ such that $\yield_1 = \yield_2 \circ \phi$.
% \end{defin}

% \david{This kind of setup assumes that a formalism allows terminal symbols to be placed anywhere that weights can be placed, and vice versa. If not, it will be a problem. For example, Chomsky normal form requires that all rules have the form $A \rightarrow BC$ or $A \rightarrow b$. If a weight is now considered a special kind of terminal symbol, then $A \rightarrow BC$ cannot have a weight.}

% Second, strong equivalence is traditionally understood to mean that two formal systems generate the same sets of structural descriptions, but this notion cannot be made precise without defining what structural descriptions are. \Citet{miller:2000} proposes relaxing this to a requirement that the sets of structural descriptions be isomorphic, in the sense of preserving certain functions or relations. But he leaves open what those preserved functions and relations are. Here, we use \cref{def:isomorphism}.
% \begin{defin}
% Two formal systems $(\carrierset_1, \yield_1)$ and $(\carrierset_2, \yield_2)$ over the same monoid are \defn{\topeqJJ} if there is an isomorphism $\phi : \carrierset_1 \rightarrow \carrierset_2$ such that $\yield_1 = \yield_2 \circ \phi$.
% \end{defin}

% We show in \cref{app:context-free-fs} how CFGs and PDAs can be defined as formal systems using \cref{def:formal-system}. 
% CFGs and PDAs cannot be \topeqJJ{} because their derivation trees have different shapes: CFG derivation trees are branching, while PDA derivation trees are monadic (every node has at most one child).

% \begin{example}
% A context-free grammar is a formal system $\grammar$ with the carrier set $D = N \times \Sigma^*$ and the signature $\signature$ containing a $k$-ary operation for each production with $k$ nonterminals on the right-hand side. Assume the grammar is in Chomsky normal form. If $\pi$ names a production $A \rightarrow BC$, then
% \begin{equation*}
% \pi^{\grammar}((\ntvar{B}, w), (\ntvar{C}, v)) = (\ntvar{A}, wv)
% \end{equation*}
% while if $\pi$ names a production $\ntvar{A} \rightarrow \symvar{b}$, then
% \begin{equation*}
% \pi^{\grammar}() = (\ntvar{A}, \symvar{b}).
% \end{equation*}
% The yield function maps $(\ntvar{S}, w)$ to $w$.
% \end{example}

% \begin{example}
% A pushdown automaton is a formal system $\pushdown$ with carrier set $\carrierset = \kleene{\alphabet} \times \states \times \kleene{\stackalphabet}$. A derivation has the form $(u, q, \stackseq)$, where $u$ is the consumed input, $q$ is a state, and $\stackseq$ is the stack. The signature contains a nullary operation $\iota$ such that
% \begin{equation*}
% \iota^\pushdown() = (\epsilon, q_0, \epsilon)
% \end{equation*}
% And for each transition $\pi = (q, \stackseq' \xrightarrow{\symvar{a}} r, \stackseq'')$, there is a unary operation
% \begin{equation*}
% \pi^\pushdown(u, q, \stackseq \stackseq') = (ua, r, \stackseq \stackseq'').
% \end{equation*}
% The yield function maps $(w, q, \stackseq)$, where $q$ is final, to $w$.
% \end{example}

% CFGs and PDAs cannot be \topeqJJ{} because their derivation trees have different shapes: CFG derivation trees are branching, while PDA derivation trees are monadic (every node has at most one child).

Currently we give separate definitions of derivation for all four control formalisms. But it would be a lot better to give a single definition of derivation.
\begin{itemize}
\item This would generalize for free to $\mathcal{L}_3$, $\mathcal{L}_4$, etc.
\item If we show that CFG is d-weakly equivalent to PDA, then hopefully it would follow immediately that CFG $\control$ X is d-weakly equivalent to PDA $\control$ X, and X $\control$ CFG is d-weakly equivalent to X $\control$ PDA.
\end{itemize}

I think doing this properly may need two major changes.

First, the definition of derivation (and d-strong equivalence) needs to be modified so that a derivation records which step yields each terminal symbol.\david{I forgot why?} Something like
\begin{defin}
A \defn{derivation} is a (unordered, unlabeled) tree $t$ together with a string $\str$ and mapping $d$ from the positions of $\str$ to the nodes of $t$.\alexandra{I think we should add the fact that a node labeled with $\ell_1$ has a child labeled with $\ell_2$ if $\ell_2$ can be applied immediately after $\ell_1$}
\end{defin}
This is similar to the definition of an indexed string by \citet{becker-etal-1992-derivational}, but maps string positions to tree nodes instead of natural numbers.
\begin{example}
\begin{align*}
\grammar_1 &= \left\{\begin{aligned} 
\ell_1 &: \sym{S}_1 \rightarrow \sym{S}_1 \sym{(} \dist{\sym{S}}_1 \sym{)} \\
\ell_2 &: \sym{S}_1 \rightarrow \varepsilon
\end{aligned} \right\}
&
\grammar_2 &= \left\{\begin{aligned}
L_1 &: \sym{S}_2 \rightarrow \ell_1 \ell_1 \sym{S}_2 \\
L_2 &: \sym{S}_2 \rightarrow \ell_2
\end{aligned}\right\}.
\end{align*}
One derivation of $\grammar_1$ for the string $\sym{(())(())}$ is
\begin{center}
\Tree [.$\ell_1[5,8]$ [.$\ell_1[1,4]$ $\ell_2$ [.$\ell_1[2,3]$ $\ell_2$ $\ell_2$ ] ] [.$\ell_1[6,7]$ $\ell_2$ $\ell_2$ ] ]
\end{center}
where $\ell_1[5,8]$ stands for a usage of production $\ell_1$ that yields the 5th and 8th symbols of the string, and similarly for the other derivation steps.

The sole derivation of $\grammar_2$ for the string $\ell_1\ell_1\ell_2$ is
\begin{center}
\Tree [.$L_1[1,2]$ $L_2[3]$ ]
\end{center}
\end{example}

In Weir's definition, a controlled grammar builds a control word by recording which productions are used, and only at the end of the derivation are the control words checked for membership in the control grammar's language. This isn't very convenient for thinking about derivations of the combined grammar. Here's an alternative definition.

For simplicity of notation, we assume that CFG production right-hand sides have either all nonterminal symbols (including one distinguished nonterminal, in LD-CFG) or a lone terminal symbol. Similarly, we assume that PDA transitions either scan $\varepsilon$ (and push one distinguished nonterminal, in LD-PDA) or push $\varepsilon$. There shouldn't be any loss of generality, but I'm not sure yet how much more complex the notation for the general case would be.

A configuration of a CFG is just a nonterminal symbol. A production either scans a terminal symbol, or can apply to a parent configuration to yield a tuple of child configurations.

A configuration of a PDA is, as usual, a state together with a stack. A transition either scans a terminal symbol, or can apply to a parent configuration to yield a child configuration.

A configuration of an LD-CFG is $\ntvar{X}[\NTvar{C}]$ where $\ntvar{X}$ is a nonterminal symbol of the LD-CFG and $\NTvar{C}$ is a configuration of the controller.
To get from a parent configuration $\ntvar{X}[\NTvar{C}]$ to a tuple of child configurations, one of the following happens: (a) In the controller, $\NTvar{C} \Rightarrow \NTvar{C'}$ scans $\ell$, and in the controllee, $\ntvar{X} \xRightarrow{\ell} \ntvar{Y}_1, \ldots, \ntvar{Y}_k$. (b) In the controllee, $\ntvar{X} \xRightarrow{\ell} \symvar{a}$. (c) In the controller, $\NTvar{C} \Rightarrow \NTvar{C'}$ scans $\varepsilon$.

A configuration of an LD-PDA is $q, \ntvar{X}_1[\NTvar{C}_1] \cdots \ntvar{X}_n[\NTvar{C}_n]$ where each $\ntvar{X}_i$ is a stack symbol of the LD-PDA and each $\NTvar{C}$ is a configuration of the controller. still writing

\subsection{CFG $\control$ CFG}

The terminals of the controller CFG can be eliminated by replacing them with the corresponding productions of the controllee. If the controller has a production $\NTvar{A}\rightarrow \Symvar{\ell}$ and the LD-CFG has a production $\Symvar{\ell} \colon \ntvar{X} \rightarrow \ntvar{Y}_1 \ldots \ntvar{\dist{Y}}_d \ldots \ntvar{Y}_k$, they can be merged into the following rule
\[
\NTvar{A}\rightarrow
\begin{tikzpicture}[baseline=0]
    \Tree [.{$\ntvar{X}$} {${\ntvar{Y}_1}\subst$} \edge[draw=none]; {$\ldots$} {${\ntvar{\dist{Y}}_d}\foot$} \edge[draw=none]; {$\ldots$} {${{\ntvar{Y}_k}\subst}$} ]
\end{tikzpicture}
\] \david{I'm confused, why are we converting to a TAG?}
The controllee's nonterminal on the lhs becomes the root of the tree on rhs of the new rules and the nonterminals on the rhs become its children. The distinguished nonterminal becomes a foot node. In general, the production of the controllee can contain a sequence of terminal and nonterminal symbols (one of which is distinguished). Therefore, the tree resulting from such a rule can have frontier nodes that are labeled with both terminals and nonterminals. 

In normal form, the productions of the controller of type $\NTvar{A}\rightarrow \NTvar{B}_1 \ldots \NTvar{B}_k$ need to be converted into the following two types of tree adjoining rules:
\[
\NTvar{A}\rightarrow
\begin{tikzpicture}[baseline=0]
    \Tree [.{$\NTvar{B}_1$} [.{$\vdots$} [.{${\NTvar{B}_k}\foot$} ] ] ]
\end{tikzpicture}
\qquad
\NTvar{A}\rightarrow
\begin{tikzpicture}[baseline=0]
    \Tree [.{$\NTvar{B}_1$} [.{$\vdots$} [.{${\NTvar{B}_k}\subst$} ] ] ]
\end{tikzpicture}
\]
In general, a production of the controller can generate a sequence of terminals and nonterminals. When this is the case, all the trees resulting from LD-CFG rules labeled with those terminals must be merged into a single tree. The trees are chained by attaching the root of a tree to the foot of the previous tree. In doing so, the new tree can have nodes labeled with multiple symbols, which can be both nonterminals of the controllee and of the controller. A derived tree will only be valid if every node is labeled with at most two matching symbols. This resembles the derivation process of feature structure-based TAG \cite{vijay-shanker-joshi-1988-feature}.

\begin{example}
    Consider a slightly modified version of the controller CFG from \cref{ex:derivations}:
    \begin{align*}
        \NT{S}_2 &\rightarrow \NT{T} \Sym{\ell}_3, \\
        \NT{T} &\rightarrow \Sym{\ell}_1 \NT{T} \Sym{\ell}_2, \\
        \NT{T} &\rightarrow \varepsilon, \\
        \NT{S}_2 &\rightarrow \Sym{\ell}_i, \quad (i=4,\ldots,7).
    \end{align*}
    The production rules resulting from merging the productions of this controller CFG with the productions of the LD-CFG from \cref{ex:derivations} are the following:
    \[
    \NTvariii{T}{S_1}{S_1} \rightarrow
    \begin{tikzpicture}[baseline=0, level 2/.style={level distance=\normalbaselineskip}, level 3/.style={level distance=\normalbaselineskip}]
    \Tree [.$\nt{S}_1$ ${\NTvariii{A}{S_2}{}}\subst$ [.$\nt{S}_1$ \edge[draw=none]; [.$\NTvariii{T}{S_1}{S_1}$ \edge[draw=none]; [.$\nt{S}_1$ ${\NTvariii{B}{S_2}{}}\subst$ ${\nt{S}_1}\foot$ ${\NTvariii{C}{S_2}{}}\subst$ ] ] ] ${\NTvariii{D}{S_2}{}}\subst$ ] 
    \end{tikzpicture}
    \]
    \[
    \NTvariii{S_2}{S_1}{} \rightarrow
    \begin{tikzpicture}[baseline=0, level 1/.style={level distance=\normalbaselineskip}]
    \Tree [.$\NTvariii{T}{S_1}{S_1}$ \edge[draw=none]; [.$\nt{S}_1$ $\varepsilon$ ] ] 
    \end{tikzpicture}
    \quad
    \NTvariii{T}{S_1}{S_1} \rightarrow \varepsilon 
    \quad
    \NTvariii{A}{S_2}{} \rightarrow
    \begin{tikzpicture}[baseline=0]
    \Tree [.$\nt{A}$
    $\sym{a}$ ] 
    \end{tikzpicture}
    \]
    \[
    {\NTvariii{B}{S_2}{}} \rightarrow
    \begin{tikzpicture}[baseline=0]
    \Tree [.$\nt{B}$
    $\sym{b}$ ] 
    \end{tikzpicture}
    \quad
    {\NTvariii{C}{S_2}{}} \rightarrow
    \begin{tikzpicture}[baseline=0]
    \Tree [.$\nt{C}$
    $\sym{c}$ ] 
    \end{tikzpicture}
    \quad
    {\NTvariii{D}{S_2}{}} \rightarrow
    \begin{tikzpicture}[baseline=0]
    \Tree [.$\nt{D}$
    $\sym{d}$ ] 
    \end{tikzpicture}
    \]
\end{example}
\alexandra{TODO: need to explain the double annotations}

\subsection{PDA $\control$ CFG}

In normal form, a transition of the controller PDA can only pop a stack symbol and scan an input symbol (label of the controllee) or pop a stack symbol and push a sequence of stack symbols, but not both. A general controller PDA can both scan a symbol and push a sequence of stack symbols. Therefore, when a controller transition scans an input symbol, it simultaneously applies the corresponding LD-CFG production. The controller configuration that is currently attached to a controllee nonterminal gets modified and passed to another nonterminal (the distinguished nonterminal) in the same step. 

\begin{example}
Consider a modified version of the controller PDA from \cref{ex:derivations}:
    \begin{align*}
        p, \NT{S}_2 &\xrightarrow{\varepsilon} p, \NT{T} \NT{L}_3 \\
        p, \NT{T} &\xrightarrow{\Sym{\ell}_1} p, \NT{T} \NT{L}_2 \\
        p, \NT{T} &\xrightarrow{\varepsilon} p, \varepsilon \\
        p, \NT{L}_2 &\xrightarrow{\Sym{\ell}_2} p, \varepsilon \\
        p, \NT{L}_3 &\xrightarrow{\Sym{\ell}_3} p, \varepsilon
    \end{align*}
    When the controller takes the second transition, the top $\NTvar{T}$ is popped from stack of the current nonterminal and is replaced with $\NT{T} \NT{L}_2$ while applying the production $\Sym{\ell_1}$ of the controllee.
\end{example}

\subsection{PDA $\control$ PDA}

\subsection{CFG $\control$ PDA}

==> main/control-formalisms.tex <==
\section{Control Formalisms}
 We extend Weir's control mechanism by allowing PDAs both as controller and controlled formalisms. We describe four \bijeqJJ{} formalisms that characterize $\tal{}$ obtained by mixing a controller CFG or PDA with an LD-CFG or LD-PDA.

\subsection{CFG $\control$ CFG}
Weir describes how to derive strings over $\tal{}$ using the productions of LD-CFGs  and the controller CFGs. We give an alternative definition\david{This ``alternative definition'' is really halfway to TAG; why not just use the definition we already established, and treat the construction here as part of the proof of equivalence to TAG?} for a derivation in a LD-CFG controlled by a CFG, which mixes the production rules of the two grammars into a single one. In doing so, we obtain a tree-generating formal system. For simplicity, we assume that the LD-CFG and the controller CFG are in normal form.

Each production in the controlled LD-CFG, $\ntvar{X}\rightarrow \sent_1\cdots\sent_k$ where $\sent_i\in \alphabet\cup\nonterm\cup\dist{\nonterm}$, can be converted into a tree that has the nonterminal $\ntvar{X}$ as root and each $\sent_i$ is a child of $\ntvar{X}$. If $\sent$ contains a distinguished nonterminal $\ntvar{Y}$, we denote it by $\kleene{\ntvar{Y}}$ and we call it a \defn{foot node}. We show in \cref{fig:ld-cfg-rules-tree-notation} how the productions of an LD-CFG in normal form can be written in tree notation.

\begin{figure}[!h]
\centering
\footnotesize
\begin{subfigure}[b]{0.15\textwidth}
\centering
$\Symvar{\ell} \colon$
\Tree [.{$\ntvar{X}$} {$\ntvar{Y}^*$} {$\ntvar{Z}$} ]
\end{subfigure}
\begin{subfigure}[b]{0.15\textwidth}
\centering
$\Symvar{\ell} \colon$
\Tree [.{$\ntvar{X}$} {$\ntvar{Y}$} {$\ntvar{Z}^*$} ]
\end{subfigure}
\begin{subfigure}[b]{0.15\textwidth}
\centering
$\Symvar{\ell} \colon$
\Tree [.{$\ntvar{X}$} {$\ntvar{Y}^*$} ]
\end{subfigure}
\begin{subfigure}[b]{0.15\textwidth}
\centering
$\Symvar{\ell} \colon$
\Tree [.{$\ntvar{X}$} {$\symvar{a}$} ]
\end{subfigure}
\begin{subfigure}[b]{0.15\textwidth}
\centering
$\Symvar{\ell} \colon$
\Tree [.{$\ntvar{X}$} {$\varepsilon$} ]
\end{subfigure}
\caption{LD-CFG production rules in tree notation.}
\label{fig:ld-cfg-rules-tree-notation}
\end{figure}

Similarly, each production in the controller CFG, $\NTvar{A}\rightarrow\sent_1\cdots\sent_k$, can be converted into a tree-rewriting rule $\NTvar{A}\rightarrow\tau$, where $\tau$ is a monadic tree with $\sent_1$ as the root and $\sent_k$ as the foot. If the controller is in normal form, we obtain the rules shown in \cref{fig:controller-cfg-rules-tree-notation}.

\begin{figure}[!h]
\centering
\footnotesize
\begin{subfigure}[b]{0.11\textwidth}
\centering
$\NTvar{A} \rightarrow$
\Tree [.{$\NTvar{B}$} {$\NTvar{C}^*$} ]
\end{subfigure}
\begin{subfigure}[b]{0.11\textwidth}
\centering
$\NTvar{A} \rightarrow$
\Tree [.{$\NTvar{B}^*$} ]
\end{subfigure}
\begin{subfigure}[b]{0.11\textwidth}
\centering
$\NTvar{A} \rightarrow \Symvar{\ell}$
\end{subfigure} 
\begin{subfigure}[b]{0.11\textwidth}
\centering
$\NTvar{A} \rightarrow \varepsilon$
\end{subfigure} 
\caption{Controller CFG rules in tree notation.}
\label{fig:controller-cfg-rules-tree-notation}
\end{figure}

The terminals of the controller (which are the labels of the controlled LD-CFG) appear only in the rule $\NTvar{A} \rightarrow \Symvar{\ell}$. 
Since, whenever the controller uses this rule, the controlled LD-CFG uses a rule labeled~$\ell$,
we substitute the trees of the controlled LD-CFG into $\NTvar{A} \rightarrow \Symvar{\ell}$, resulting in the rules \labelcrefrange{fig:rules-tag-cnf-4}{fig:rules-tag-cnf-8} from \cref{fig:rules-tag-canonical-2-form}. We show in \cref{fig:rules-tag-canonical-2-form} the types of rules that can be obtained from an LD-CFG controlled by a CFG when both grammars are in normal form. We give an example of tree rewriting rules in \cref{app:examples}.

\begin{figure}[!h]
\centering
\footnotesize
\begin{subfigure}[b]{0.2\textwidth}
\centering
$\NTvar{A} \rightarrow$
\Tree [.{$\NTvar{B}^*$} ]
\caption{}
\label{fig:rules-tag-cnf-2}
\end{subfigure}
\centering
\begin{subfigure}[b]{0.2\textwidth}
\centering
$\NTvar{A} \rightarrow \varepsilon$
\caption{}
\label{fig:rules-tag-cnf-3}
\end{subfigure} 
\begin{subfigure}[b]{0.15\textwidth}
\centering
$\NTvar{A} \rightarrow$
\Tree [.{$\NTvar{B}$} {$\NTvar{C}^*$} ]
\caption{}
\label{fig:rules-tag-cnf-1}
\end{subfigure}
\begin{subfigure}[b]{0.15\textwidth}
\centering
$\NTvar{A} \rightarrow$
\Tree [.{$\ntvar{X}$} {$\ntvar{Y}^*$} {$\ntvar{Z}$} ]
\caption{}
\label{fig:rules-tag-cnf-4}
\end{subfigure}
\begin{subfigure}[b]{0.15\textwidth}
\centering
$\NTvar{A} \rightarrow$
\Tree [.{$\ntvar{X}$} {$\ntvar{Y}$} {$\ntvar{Z}^*$} ]
\caption{}
\label{fig:rules-tag-cnf-5}
\end{subfigure}
\begin{subfigure}[b]{0.15\textwidth}
\centering
$\NTvar{A} \rightarrow$
\Tree [.{$\ntvar{X}$} {$\ntvar{Y}^*$} ]
\caption{}
\label{fig:rules-tag-cnf-6}
\end{subfigure}
\begin{subfigure}[b]{0.15\textwidth}
\centering
$\NTvar{A} \rightarrow$
\Tree [.{$\ntvar{X}$} {$\symvar{x}$} ]
\caption{}
\label{fig:rules-tag-cnf-7}
\end{subfigure}
\begin{subfigure}[b]{0.15\textwidth}
\centering
$\NTvar{A} \rightarrow$
\Tree [.{$\ntvar{X}$} {$\varepsilon$} ]
\caption{}
\label{fig:rules-tag-cnf-8}
\end{subfigure}
\caption{Rules of CFG $\control$ CFG in normal form.}
\label{fig:rules-tag-canonical-2-form}
\end{figure}

% \begin{figure}[!h]
% % \centering
% \footnotesize
% \begin{subfigure}[b]{0.15\textwidth}
% $\NTvar{A} \rightarrow$
% \Tree [.{$\NTvar{B}$} {$\NTvar{C}^*$} ]
% \caption{}
% \end{subfigure}
% \begin{subfigure}[b]{0.15\textwidth}
% $\NTvar{S} \rightarrow \varepsilon$
% \caption{}
% \end{subfigure} 
% \begin{subfigure}[b]{0.15\textwidth}
% $\NTvar{A} \rightarrow$
% \Tree [.{$\ntvar{X}$} {$\ntvar{Y}^*$} {$\ntvar{Z}$} ]
% \caption{}
% \end{subfigure}
% \begin{subfigure}[b]{0.15\textwidth}
% $\NTvar{A} \rightarrow$
% \Tree [.{$\ntvar{X}$} {$\ntvar{Y}$} {$\ntvar{Z}^*$} ]
% \caption{}
% \end{subfigure}
% \begin{subfigure}[b]{0.15\textwidth}
% $\NTvar{A} \rightarrow$
% \Tree [.{$\ntvar{X}$} {$\symvar{x}$} ]
% \caption{}
% \end{subfigure}
% \begin{subfigure}[b]{0.15\textwidth}
% $\NTvar{A} \rightarrow$
% \Tree [.{$\ntvar{S}$} {$\varepsilon$} ]
% \caption{}
% \end{subfigure}
% \caption{General rules of an LD-CFG controlled by a CFG in CNF.}
% \label{fig:rules-tag-cnf}
% \end{figure}
\alexandra{not sure how to justify the presence of an $\varepsilon$ as a node in an elementary tree. \response{david} me neither. is the epsilon rule absolutely necessary?}
\begin{defin}
Let $\grammar$ be an LD-CFG with nonterminals $\nonterm$ and terminals $\alphabet$. A tree $\tau$ is called \defn{elementary} if all its nodes are labeled either with symbols from $\nonterm$ or $\alphabet$. 
\end{defin}
\alexandra{should we give also a formal definition of an LD-CFG controlled by a CFG similar to TAG?}
% A tree $\tau'$ can be obtained from a tree $\tau$ by applying a production rule $p$ to one of $\tau$'s nodes. We reuse the notation $\tau \xRightarrow{p}\tau'$ defined in the context of TAG. 
\david{currently in appendix}
A production $\ntvar{X}\rightarrow\tau$ can be applied to any $\ntvar{X}$-labeled node in a tree by \emph{adjoining} $\tau$ at that node, if $\tau$ has a foot node. Otherwise, it can only be substituted by the right-hand side of the rule. We use the notation $\tau\xRightarrow{p}\tau'$ for a tree $\tau'$ derived from a tree $\tau$ using a rule $p$. We explain the adjunction operation in \cref{app:tal}.

\david{is it necessary to re-define derivation, run, etc. for the control formalisms? i would hope that it could be done once when defining what control is, then not done again for the particular control formalisms.}
\begin{defin}
A \defn{derivation} in an LD-CFG $\grammar_1$ controlled by a CFG $\grammar_2$ is a sequence of trees and productions $\derivation = \tau_0,p_1,\tau_1,\ldots,p_n,\tau_n$, where the initial tree is $\tau_0=\NTvar{S}$, $\tau_n$ is an elementary tree and, for each $i\in\range{1}{n}$, $\tau_{i-1}\xRightarrow{p_i}\tau_i$.
\end{defin}
We show an example of a derivation in \cref{app:examples}.

\begin{defin}
Let $\grammar_1$ be an LD-CFG and $\grammar_2$ a controller CFG. The \defn{string language} generated by $\grammar_1$ controlled by $\grammar_2$ is the set of strings yielded by the elementary trees derived by $\grammar_1$ controlled by~$\grammar_2$.
\end{defin}

\begin{proposition}
A CFG $\control$ CFG is \topeqJJ{} to a TAG.
\end{proposition}

% \begin{proof}
%     See \cref{app:d-strong-eq}
% \end{proof}

% \begin{figure*}
% \ContinuedFloat
%     \centering
%     \begin{subfigure}[b]{0.25\textwidth}
%         \centering
%         \Tree [.{$\nt{S_1}$} [.{$\nt{A}$} {$a$} ] [.{$\nt{S_1}$} [.{$\nt{S_1}$} [.{$\nt{S_1}$} {$\nt{B}$} [.{$\NT{T}$} [.{$\NT{L_4}$} [.{$\nt{S_1}$} [.{$\nt{S_1}$} {$\varepsilon$} ] [.{$\nt{A}$} {$a$} ] ] ] ] ] ] ] ]
%         $ \quad \Rightarrow$
%      \end{subfigure}
%      \begin{subfigure}[b]{0.25\textwidth}
%         \centering
%         \Tree [.{$\nt{S_1}$} [.{$\nt{A}$} {$a$} ] [.{$\nt{S_1}$} [.{$\nt{S_1}$} [.{$\nt{S_1}$} [.{$\nt{B}$} {$b$} ] [.{$\NT{T}$} [.{$\NT{L_4}$} [.{$\nt{S_1}$} [.{$\nt{S_1}$} {$\varepsilon$} ] [.{$\nt{A}$} {$a$} ] ] ] ] ] ] ] ]
%         $ \quad \Rightarrow$
%      \end{subfigure}
%      \begin{subfigure}[b]{0.25\textwidth}
%         \centering
%         \Tree [.{$\nt{S_1}$} [.{$\nt{A}$} {$a$} ] [.{$\nt{S_1}$} [.{$\nt{S_1}$} [.{$\nt{S_1}$} [.{$\nt{B}$} {$b$} ] [.{$\NT{T}$} [.{$\nt{S_1}$} [.{$\nt{S_1}$} [.{$\nt{S_1}$} [.{$\NT{S_1}$} {$\varepsilon$} ] [.{$\nt{A}$} {$a$} ] ] ] ] {$\nt{B}$} ] ] ] ] ]
%         $ \quad \Rightarrow$
%      \end{subfigure}
%      \begin{subfigure}[b]{0.2\textwidth}
%         \centering
%         \Tree [.{$\nt{S_1}$} [.{$\nt{A}$} {$a$} ] [.{$\nt{S_1}$} [.{$\nt{S_1}$} [.{$\nt{S_1}$} [.{$\nt{B}$} {$b$} ] [.{$\NT{T}$} [.{$\nt{S_1}$} [.{$\nt{S_1}$} [.{$\nt{S_1}$} [.{$\nt{S_1}$} {$\varepsilon$} ] [.{$\nt{A}$} {$a$} ] ] ] ] [.{$\nt{B}$} {$b$} ] ] ] ] ] ]
%      \end{subfigure}
%     \caption{Example of derivation in a LD-CFG controlled by a CFG in tree notation.}
%     \label{fig:tag-derivation}
% \end{figure*}

\subsection{PDA $\control$ CFG}

% The following definition is the normal form for top-down PDAs from \cite{butoi+al.emnlp22}, which we call CNF here to distinguish it from the normal form:
% \david{This seems more relaxed than Chomsky normal form, so I don't know if I agree with this terminology.}
% \begin{defin}
% A controller top-down PDA is in Chomsky Normal Form if its transitions have the following form:
% \begin{align*}
% p, \NTvar{S} &\xrightarrow{\varepsilon} q, \varepsilon  \\
% p, \NTvar{A} &\xrightarrow{\varepsilon} q, \NTvar{B} \NTvar{C} \\
% p, \NTvar{A} &\xrightarrow{\Symvar{a}} q, \NTvar{B} \NTvar{C} \\
% p, \NTvar{A} &\xrightarrow{\Symvar{a}} q, \NTvar{B} \\
% p, \NTvar{A} &\xrightarrow{\Symvar{a}} q, \varepsilon
% \end{align*}
% \end{defin}

% \begin{defin}
% A controller top-down PDA is in normal form if its transitions have the following form: 
% \begin{align*}
% p, \NTvar{A} &\xrightarrow{\varepsilon} q, \NTvar{B} \NTvar{C} \\
% p, \NTvar{A} &\xrightarrow{\Symvar{a}} q, \NTvar{B} \NTvar{C} \\
% p, \NTvar{A} &\xrightarrow{\varepsilon} q, \NTvar{B} \\
% p, \NTvar{A} &\xrightarrow{\Symvar{a}} q, \NTvar{B} \\
% p, \NTvar{A} &\xrightarrow{\varepsilon} q, \varepsilon \\
% p, \NTvar{A} &\xrightarrow{\Symvar{a}} q, \varepsilon
% \end{align*}
% \end{defin}
The production rules in an LD-CFG and the transitions in a controller PDA can be merged into a single grammar by augmenting the nonterminals of the LD-CFG with PDA configurations. We assume for simplicity that both the LD-CFG and the controller PDA are in normal form.

\begin{defin}
A \defn{sentential form} $\sent$ of an LD-CFG $\grammar$ controlled by a PDA $\pushdown$ is a sequence of terminals and nonterminals of $\grammar$, in which each nonterminal is augmented with a configuration of $\pushdown$.
\end{defin}

The scanning transitions in the controller PDA \textit{control} which rules in the LD-CFG are applied in a derivation: when the controller PDA scans a terminal symbol $\Sym{\ell}$, rule $\Sym{\ell}$ in the LD-CFG is applied simultaneously. From this perspective, there are two types of rules in an LD-CFG controlled by a PDA, depending on whether the PDA's transition is scanning or non-scanning. 

A non-scanning transition of the PDA changes the configuration of a nonterminal without applying any production in the LD-CFG. If $p,\NTvar{A}\xrightarrow{\varepsilon}q,\stackseq$ is a transition $\atrans$ of the controller, a sentential form $\sent\,\ntvar{X}[p,\stackseq'\NTvar{A}]\,\sent'$ derives the sentential form $\sent\,\ntvar{X}[q,\stackseq'\stackseq]\,\sent'$. We denote this by $\sent\,\ntvar{X}[p,\stackseq'\NTvar{A}]\,\sent'\xRightarrow{\atrans}\sent\,\ntvar{X}[q,\stackseq'\stackseq]\,\sent'$. If the PDA is in normal form, we get the productions \Crefrange{eq:ldcfg-pda-rules-2-nf-10}{eq:ldcfg-pda-rules-2-nf-12} from \cref{fig:ldcfg-pda-rules-2-nf}.

A transition that scans an $\Symvar{\ell}$ changes the configuration of a nonterminal and passes it to the distinguished nonterminal on the right-hand side of a rule labeled with $\Symvar{\ell}$. Each other nonterminal on the right-hand side of $\ell$ is augmented with the PDA's initial configuration. For a sequence of nonterminals $\sent=\sent_1\ldots\sent_n$, we use the notation $\sent[q_\init,\NTvar{S}]=\sent_1[q_\init,\NTvar{S}]\ldots\sent_n[q_\init,\NTvar{S}]$. If $p, \NTvar{A}\xrightarrow{\ell}q,\varepsilon$ is a transition $\atrans$ of the controller and $\ell\colon \ntvar{X}\rightarrow\boldsymbol{\beta}\dist{\ntvar{X'}}\boldsymbol{\beta'}$ is a production of the LD-CFG, a sentential form $\sent\,\ntvar{X}[p,\stackseq\NTvar{A}]\,\sent'$ derives the sentential form $\sent\,\boldsymbol{\beta}[q_\init,\NTvar{S}]\,\ntvar{X'}[q,\stackseq]\,\boldsymbol{\beta}[q_\init,\NTvar{S}]\,\sent'$. We denote this by $\sent\,\ntvar{X}[p,\stackseq\NTvar{A}]\,\sent'\xRightarrow{\ell}\sent\,\boldsymbol{\beta}[q_\init,\NTvar{S}]\,\ntvar{X'}[q,\stackseq]\,\boldsymbol{\beta}[q_\init,\NTvar{S}]\,\sent'$. By mixing these rules of an LD-CFG and a controller PDA in normal form we get the types of productions \Crefrange{eq:ldcfg-pda-rules-2-nf-7}{eq:ldcfg-pda-rules-2-nf-14} from \cref{fig:ldcfg-pda-rules-2-nf}. We use two types of arrows to distinguish between the scanning and non-scanning transitions of the controller. When the transition is non-scanning, we use an arrow of the type $\rightarrow$ and when the transition is scanning (which implies that we apply also a rule of the LD-CFG) we use an arrow of the type $\outarrow$.

% Similarly, \cref{fig:ldcfg-pda-rules-cnf} shows the productions when the LD-CFG and the controller PDA are in CNF.

\begin{figure}[!h]
\footnotesize
\begin{align}
    \ntvar{X} [p, \rest \NTvar{A}] &\rightarrow \ntvar{X} [q, \rest \NTvar{B} \NTvar{C}] \label{eq:ldcfg-pda-rules-2-nf-10} \\
    \ntvar{X} [p, \rest \NTvar{A}] &\rightarrow \ntvar{X} [q, \rest \NTvar{B}]  \label{eq:ldcfg-pda-rules-2-nf-11} \\
    \ntvar{X} [p, \rest \NTvar{A}] &\rightarrow \ntvar{X} [q, \rest] \label{eq:ldcfg-pda-rules-2-nf-12} \\
    % \ntvar{X} [p, \rest \NTvar{A}] &\outarrow \ntvar{Y} [q, \rest \NTvar{B} \NTvar{C}] \ntvar{Z} [q_0, \NTvar{S}] \label{eq:ldcfg-pda-rules-2-nf-1} \\
    % \ntvar{X} [p, \rest \NTvar{A}] &\outarrow \ntvar{Y} [q_0, \NTvar{S}] \ntvar{Z} [q, \rest \NTvar{B} \NTvar{C}]  \label{eq:ldcfg-pda-rules-2-nf-2} \\
    % \ntvar{X} [p, \rest \NTvar{A}] &\outarrow \ntvar{Y} [q, \rest \NTvar{B} \NTvar{C}]  \label{eq:ldcfg-pda-rules-2-nf-3} \\
    % \ntvar{X} [p, \rest \NTvar{A}] &\outarrow \ntvar{Y} [q, \rest \NTvar{B}] \ntvar{Z} [q_0, \NTvar{S}]  \label{eq:ldcfg-pda-rules-2-nf-4} \\
    % \ntvar{X} [p, \rest \NTvar{A}] &\outarrow \ntvar{Y} [q_0, \NTvar{S}] \ntvar{Z} [q, \rest \NTvar{B}] \label{eq:ldcfg-pda-rules-2-nf-5} \\
    % \ntvar{X} [p, \rest \NTvar{A}] &\outarrow \ntvar{Y} [q, \rest \NTvar{B}]  \label{eq:ldcfg-pda-rules-2-nf-6} \\
    \ntvar{X} [p, \rest \NTvar{A}] &\outarrow \ntvar{Y} [q, \rest] \ntvar{Z} [q_\init, \NTvar{S}]  \label{eq:ldcfg-pda-rules-2-nf-7} \\
    \ntvar{X} [p, \rest \NTvar{A}] &\outarrow \ntvar{Y} [q_\init, \NTvar{S}] \ntvar{Z} [q, \rest]  \label{eq:ldcfg-pda-rules-2-nf-8} \\
    \ntvar{X} [p, \rest \NTvar{A}] &\outarrow \ntvar{Y} [q, \rest]  \label{eq:ldcfg-pda-rules-2-nf-9} \\
    \ntvar{X} [p, \NTvar{A}] &\outarrow \varepsilon \label{eq:ldcfg-pda-rules-2-nf-13} \\
    \ntvar{X} [p, \NTvar{A}] &\outarrow \symvar{a} \label{eq:ldcfg-pda-rules-2-nf-14}
\end{align}
\caption{Rules of PDA $\control$ CFG in normal form.}
\label{fig:ldcfg-pda-rules-2-nf}
\end{figure}

% \begin{figure}[!h]
% \footnotesize
% \begin{align*}
% \ntvar{X} [p, \rest \NTvar{A}] &\outarrow \ntvar{Y} [q, \rest \NTvar{B} \NTvar{C}] \ntvar{Z} [s, \NTvar{S}]  &\text{inside \& outside} \\
% \ntvar{X} [p, \rest \NTvar{A}] &\outarrow \ntvar{Y} [s, \NTvar{S}] \ntvar{Z} [q, \rest \NTvar{B} \NTvar{C}] &\text{inside \& outside} \\
% \ntvar{X} [p, \rest \NTvar{A}] &\outarrow \ntvar{Y} [q, \rest \NTvar{B}] \ntvar{Z} [s, \NTvar{S}] &\text{inside \& outside} \\
% \ntvar{X} [p, \rest \NTvar{A}] &\outarrow \ntvar{Y} [s, \NTvar{S}] \ntvar{Z} [q, \rest \NTvar{B}] &\text{inside \& outside} \\
% \ntvar{X} [p, \rest \NTvar{A}] &\outarrow \ntvar{Y} [q, \rest] \ntvar{Z} [s, \NTvar{S}] &\text{inside \& outside} \\
% \ntvar{X} [p, \rest \NTvar{A}] &\outarrow \ntvar{Y} [s, \NTvar{S}] \ntvar{Z} [q, \rest] &\text{inside \& outside} \\
% \ntvar{X} [p, \rest \NTvar{A}] &\rightarrow \ntvar{X} [q, \rest \NTvar{B} \NTvar{C}] &\text{inside} \\
% \ntvar{S} [p, \NTvar{A}] &\outarrow \varepsilon &\text{inside \& outside} \\
% \ntvar{X} [p, \NTvar{A}] &\outarrow a &\text{inside \& outside}
% \end{align*}
% \caption{Production rules of a LD-CFG controlled by a PDA in CNF.}
% \label{fig:ldcfg-pda-rules-cnf}
% \end{figure}
\begin{defin}
A \defn{derivation} in an LD-CFG $\grammar$ controlled by a PDA $\pushdown$ is a sequence of sentential forms and productions $\derivation=\sent_0,p_1,\sent_1,\ldots,p_n,\sent_n$, where $\sent_0=\ntvar{S}[q_\init,\NTvar{S}]$, $\sent_{i-1}\xRightarrow{p_i}\sent_i$ for $i\in \range{1}{n}$. We say that $\grammar$ controlled by $\pushdown$ \defn{derives} the string $\sent_n$. The \defn{language} of $\grammar$ controlled by $\pushdown$ is the set of strings they derive.
\end{defin}

\cref{fig:ldcfg-pda-derivation} shows a derivation in a PDA $\control$ CFG.
\begin{figure}[!h]
\centering
\footnotesize
\begin{align*}
\nt{S_1} [p, \NT{S_2}] &\Rightarrow \nt{S_1} [p, \NT{L_5} \NT{T}] \\
&\Rightarrow \nt{S_1} [p, \NT{L_5} \NT{L_3} \NT{L_6}] \\
&\Rightarrow \nt{S_1} [p, \NT{L_5} \NT{L_3} \NT{T} \NT{L_1}] \\
&\Rightarrow \nt{A} [p, \NTvar{S_2}] \NT{S_1} [p, \NT{L_5} \NT{L_3} \NT{T}]\\
% &\Rightarrow \nt{A} [p, \NTvar{L_5 T}] \NT{S_1} [p, \NT{L_5} \NT{L_3} \NT{T}]\\
% &\Rightarrow \nt{A} [p, \NTvar{L_5}] \NT{S_1} [p, \NT{L_5} \NT{L_3} \NT{T}]\\
&\Rightarrow^3 a \nt{S_1} [p, \NT{L_5} \NT{L_3} \NT{T}] \\
&\Rightarrow a \nt{S_1} [p, \NT{L_5} \NT{L_3} \NT{L_4} \NT{L_7}] \\
&\Rightarrow a \nt{S_1} [p, \NT{L_5} \NT{L_3} \NT{L_4} \NT{T} \NT{L_2}] \\
&\Rightarrow a \nt{B} [p, \NT{S_2}] \nt{S_1} [p, \NT{L_5} \NT{L_3} \NT{L_4} \NT{T}] \\
% &\Rightarrow a \nt{B} [p, \NT{L_5 T}] \nt{S_1} [p, \NT{L_5} \NT{L_3} \NT{L_4} \NT{T}] \\
% &\Rightarrow a \nt{B} [p, \NT{L_5}] \nt{S_1} [p, \NT{L_5} \NT{L_3} \NT{L_4} \NT{T}] \\
&\Rightarrow^3 ab \nt{S_1} [p, \NT{L_5} \NT{L_3} \NT{L_4} \NT{T}] \\
&\Rightarrow ab \nt{S_1} [p, \NT{L_5} \NT{L_3} \NT{L_4}] \\
&\Rightarrow ab \nt{S_1} [p, \NT{L_5} \NT{L_3}] \NT{B} \left[p, \NT{S_2}\right] \\
&\Rightarrow ab\nt{S_1} [p, \NT{L_5}] \nt{A} \left[p, \NT{S_2}\right] \nt{B} \left[p, \NT{S_2}\right] \\
% &\Rightarrow ab\nt{S_1} [p, \NT{L_5}] \nt{A} \left[p, \NT{S_2}\right] \nt{B} \left[p, \NT{L_5 T}\right] \\
% &\Rightarrow ab\nt{S_1} [p, \NT{L_5}] \nt{A} \left[p, \NT{S_2}\right] \nt{B} \left[p, \NT{L_5}\right] \\
&\Rightarrow ab \nt{A} \left[p, \NT{S_2}\right] \NT{B} \left[p, \NT{S_2}\right] \\
% &\Rightarrow ab \nt{A} \left[p, \NT{L_5 T}\right] \NT{B} \left[p, \NT{S_2}\right] \\
% &\Rightarrow ab \nt{A} \left[p, \NT{L_5}\right] \NT{B} \left[p, \NT{S_2}\right] \\
&\Rightarrow^3 aba \nt{B} \left[p, \NT{S_2}\right] \\
% &\Rightarrow aba \nt{B} \left[p, \NT{L_5 T}\right] \\
% &\Rightarrow aba \nt{B} \left[p, \NT{L_5}\right] \\
&\Rightarrow^3 abab
\end{align*}
\caption{Derivation in a PDA $\control$ CFG.}
\label{fig:ldcfg-pda-derivation}
\end{figure}

\begin{proposition}
A PDA $\control$ CFG is \topeqJJ{} to a LIG.
\end{proposition}

% \begin{proof}
%     See \cref{app:d-strong-eq}
% \end{proof}
% \subsubsection{Equivalence with LIG}

% \begin{theorem}
% The formal system defined by a LD-CFG controlled by a PDA is LIG.
% \end{theorem}
% \begin{proof}
%     Sketch:

%     $(\Rightarrow)$ Let $\grammar = (\nonterm, \alphabet, L, \rules, \ntvar{S})$ be an LD-CFG and $\pushdown = (\states, L, \stackalphabet, \trans, (q_i, \NTvar{S}), (q_f, \varepsilon))$ a controller PDA. We assume that $\grammar$ is in 2-Form and $\pushdown$ is a top-down PDA in normal form and we obtained the productions rules $\rules_{\trans}$ from \cref{fig:ldcfg-pda-rules-2-nf} by merging $\rules$ and $\trans$
%     We can construct a LIG $\grammar' = (\nonterm', \alphabet', \stackalphabet', \ntvar{S'}, \rules')$, where $\nonterm' = \{\ntvar{X}_p \mid \ntvar{X} \in \nonterm, p \in \states \}$, $\alphabet' = \alphabet$, $\stackalphabet' = \stackalphabet$, $\ntvar{S'} = \ntvar{S}_{q_i}$ and the set of productions $\rules'$ can be obtained by converting the rules from \cref{fig:ldcfg-pda-rules-2-nf} as follows:
%     \begin{align*}
%     \footnotesize
%     \ntvar{X_p} [\rest \NTvar{A}] &\rightarrow \ntvar{X_q} [\rest \NTvar{B} \NTvar{C}] \\
%     \ntvar{X_p} [\rest \NTvar{A}] &\rightarrow \ntvar{X_q} [\rest \NTvar{B}]  \\
%     \ntvar{X_p} [\rest \NTvar{A}] &\rightarrow \ntvar{X_q} [\rest]  \\
%     \ntvar{X_p} [\rest \NTvar{A}] &\outarrow \ntvar{Y_q} [\rest \NTvar{B} \NTvar{C}] \ntvar{Z_s} [\NTvar{S}] \\
%     \ntvar{X_p} [\rest \NTvar{A}] &\outarrow \ntvar{Y_s} [\NTvar{S}] \ntvar{Z_q} [\rest \NTvar{B} \NTvar{C}] \\  
%     \cdots
%     \end{align*}

%     $(\Leftarrow)$ Let $\grammar = (\nonterm, \alphabet, \stackalphabet, \ntvar{S}, \rules)$ be a LIG in normal form. We can construct the LD-CFG $\grammar' = (\nonterm', \alphabet', L, \rules', \ntvar{S'})$, where $\nonterm' = \nonterm$, $\alphabet' = \alphabet$ and $\ntvar{S'} = \ntvar{S}$ and rules $\rules'$
%     % \begin{align*}
%     %     \ntvar{X} &\rightarrow \dist{\ntvar{Y}} \\
%     %     \ntvar{X} &\rightarrow \dist{\ntvar{Y}} \ntvar{Z} \\
%     %     \ntvar{X} &\rightarrow \ntvar{Y} \dist{\ntvar{Z}} \\
%     %     \ntvar{X} &\rightarrow \symvar{a} \\
%     %     \ntvar{X} &\rightarrow \varepsilon.
%     % \end{align*}
%     The controller PDA is $\pushdown = (\states, L, \stackalphabet', \trans, (q_i, \NTvar{S}), (q_f, \varepsilon))$ where $\states = \{p \}$, $\stackalphabet' = \stackalphabet$, $q_i = p$ and $q_f = p$. For each transition of type $\ntvar{X} [\rest \NTvar{A}] \rightarrow \ntvar{X} [\rest \stackseq], |\stackseq| \leq 2$ in $\rules$ add a transition $p, \NTvar{A} \xrightarrow{\varepsilon} p, \stackseq$ in $\trans$. For transitions of type \Crefrange{eq:ldcfg-pda-rules-2-nf-1}{eq:ldcfg-pda-rules-2-nf-14} add a fresh label $\ell$ to $L$, a rule of one of the types shown in \cref{def:ldcfg-canonical-2f} to $\rules'$ and a transition of the form $p, \NTvar{A} \xrightarrow{\varepsilon} p, \stackseq$ to $\trans$.
% \end{proof}

\subsection{PDA $\control$ PDA}
% \subsection{Normal Forms}

% We give two normal forms for LD-PDAs that are analogous to the CNF and the normal form for LD-CFGs:

% \begin{defin}
% An LD-PDA is in Chomsky Normal Form (CNF) if its transitions are of the following form:
% \begin{align*}
% &\Symvar{\ell} \colon p, \ntvar{X} \xrightarrow[]{\varepsilon} q,  \ntvar{\dist{Y}} \ntvar{Z} \\
% &\Symvar{\ell} \colon p, \ntvar{X} \xrightarrow[]{\varepsilon} q, \ntvar{Y} \ntvar{\dist{Z}} \\
% &\Symvar{\ell} \colon p, \ntvar{X} \xrightarrow[]{\symvar{x}} q,  \ntvar{\dist{Y}} \ntvar{Z} \\
% &\Symvar{\ell} \colon p, \ntvar{X} \xrightarrow[]{\symvar{x}} q, \ntvar{Y} \ntvar{\dist{Z}} \\
% &\Symvar{\ell} \colon p, \ntvar{X} \xrightarrow[]{\symvar{x}} q,  \ntvar{\dist{Y}} \\
% &\Symvar{\ell} \colon p, \ntvar{X} \xrightarrow[]{\symvar{x}} q, \varepsilon \\
% &\Symvar{\ell} \colon p, \ntvar{S} \xrightarrow[]{\varepsilon} q, \varepsilon 
% \end{align*}
% \end{defin}

% \begin{defin}
% An LD-PDA is in normal form if its transitions are of the following form:
% \begin{align*}
% &\Symvar{\ell} \colon p, \ntvar{X} \xrightarrow[]{\varepsilon} q,  \ntvar{\dist{Y}} \ntvar{Z} \\
% &\Symvar{\ell} \colon p, \ntvar{X} \xrightarrow[]{\varepsilon} q, \ntvar{Y} \ntvar{\dist{Z}} \\
% &\Symvar{\ell} \colon p, \ntvar{X} \xrightarrow[]{\varepsilon} q,  \ntvar{\dist{Y}} \\
% &\Symvar{\ell} \colon p, \ntvar{X} \xrightarrow[]{\varepsilon} q, \varepsilon \\
% &\Symvar{\ell} \colon p, \ntvar{X} \xrightarrow[]{\symvar{x}} q,  \ntvar{\dist{Y}} \ntvar{Z} \\
% &\Symvar{\ell} \colon p, \ntvar{X} \xrightarrow[]{\symvar{x}} q, \ntvar{Y} \ntvar{\dist{Z}} \\
% &\Symvar{\ell} \colon p, \ntvar{X} \xrightarrow[]{\symvar{x}} q,  \ntvar{\dist{Y}} \\
% &\Symvar{\ell} \colon p, \ntvar{X} \xrightarrow[]{\symvar{x}} q, \varepsilon
% \end{align*}
% \end{defin}

The transitions of an LD-PDA and a controller PDA can be merged into a single set of transitions by augmenting the LD-PDA's stack symbols with configurations of the controller, similar to the rules of an LD-CFG controlled by a PDA. 

\begin{defin}
A \defn{configuration} of an LD-PDA $\pushdown_1$ controlled by a PDA $\pushdown_2$ is a pair $(p,\stackseq)$, where $p$ is the current state and $\stackseq$ is the current stack, in which each stack symbol is augmented with a configuration of $\pushdown_2$.
\end{defin}

We distinguish two types of transitions, depending on whether the controller's transition is scanning or non-scanning. The non-scanning transitions of the controller change the configuration of a stack symbol in the LD-PDA, without taking any transition in the LD-PDA. If the controller PDA is in normal form, we get the transitions \Crefrange{eq:ldpda-pda-rules-2-nf-1}{eq:ldpda-pda-rules-2-nf-3} from \cref{fig:ldpda-pda-rules-2-nf}. 
% If $\atrans=r,\NTvar{A}\xrightarrow{\varepsilon}s,\stackseq$, where $|\stackseq|\leq 2$, is a transition of the controller, and $(p,\nestedstack \ntvar{X}[r, \stackseq'\NTvar{A}])$ and $(p,\nestedstack \ntvar{X}[s, \stackseq'\stackseq])$ are configurations of the LD-PDA, we write $(p,\nestedstack \ntvar{X}[r, \stackseq'\NTvar{A}])\xRightarrow{\atrans}(p,\nestedstack \ntvar{X}[s, \stackseq'\stackseq])$.

A transition of the controller that scans $\Symvar{\ell}$ applies simultaneously a transition labeled with $\Symvar{\ell}$ in the LD-PDA. The new configuration of the controller PDA gets associated with the distinguished stack symbol in $\Symvar{\ell}$ and every other stack symbol is augmented with the controller's initial configuration. If both the LD-CFG and the controller are in normal form, we obtain the types of transitions shown in \cref{fig:ldpda-pda-rules-2-nf}, \Crefrange{eq:ldpda-pda-rules-2-nf-6}{eq:ldpda-pda-rules-2-nf-13}. 
% If $r,\NTvar{A}\xrightarrow{\ell}s,\varepsilon$ is a transition of the controller, $\ell\colon p,\ntvar{X}\xrightarrow{\langle\symvar{a},w\rangle}q,\boldsymbol{\beta}\dist{\ntvar{X'}}\boldsymbol{\beta'}$ is a transition of the LD-CFG, and $(p,\nestedstack \ntvar{X}[r,\stackseq\NTvar{A}])$ and $(q, \nestedstack \boldsymbol{\beta}[q_\init,\stackseq_\init]\ntvar{X'}[s,\stackseq]\boldsymbol{\beta'}[q_\init,\stackseq_\init])$ are configurations, we write $(p,\nestedstack \ntvar{X}[r,\stackseq\NTvar{A}])\Rightarrow (q, \nestedstack \boldsymbol{\beta}[q_\init,\stackseq_\init]\ntvar{X'}[s,\stackseq]\boldsymbol{\beta'}[q_\init,\stackseq_\init])$.

\begin{figure}[!h]
\footnotesize
\begin{align}
    p, \nestedstack \ntvar{X} [r, \rest \NTvar{A}] &\xrightarrow{\varepsilon} p, \nestedstack \ntvar{X} [s, \rest \NTvar{B} \NTvar{C}] \label{eq:ldpda-pda-rules-2-nf-1} \\
    p, \nestedstack \ntvar{X} [r, \rest \NTvar{A}] &\xrightarrow{\varepsilon} p, \nestedstack \ntvar{X} [s, \rest \NTvar{B}] \label{eq:ldpda-pda-rules-2-nf-2}\\
    p, \nestedstack \ntvar{X} [r, \rest \NTvar{A}] &\xrightarrow{\varepsilon} p, \nestedstack \ntvar{X} [s, \rest] \label{eq:ldpda-pda-rules-2-nf-3} \\
    % p, \nestedstack \ntvar{X} [r, \rest \NTvar{A}] &\xoutarrow{\varepsilon} q, \nestedstack \ntvar{Y} [s, \rest \NTvar{B} \NTvar{C}] \ntvar{Z}[s, \NTvar{S}] \label{eq:ldpda-pda-rules-2-nf-4} \\
    % p, \nestedstack \ntvar{X} [r, \rest \NT{A}] &\xoutarrow{\varepsilon} q, \nestedstack \ntvar{Y} [s, \rest \NTvar{B}] \ntvar{Z}[s, \NTvar{S}] \label{eq:ldpda-pda-rules-2-nf-5} \\
    p, \nestedstack \ntvar{X} [r, \rest \NTvar{A}] &\xoutarrow{\varepsilon} q, \nestedstack \ntvar{Y} [s, \rest] \ntvar{Z}[q_\init, \NTvar{S}] \label{eq:ldpda-pda-rules-2-nf-6} \\
    % p, \nestedstack \ntvar{X} [r, \rest \NTvar{A}] &\xoutarrow{\varepsilon} q, \nestedstack \ntvar{Y} [s, \NTvar{S}] \ntvar{Z} [s, \rest \NTvar{B} \NTvar{C}] \label{eq:ldpda-pda-rules-2-nf-7} \\
    % p, \nestedstack \ntvar{X} [r, \rest \NTvar{A}] &\xoutarrow{\varepsilon} q, \nestedstack \ntvar{Y} [s, \NTvar{S}]\ntvar{Z} [s, \rest \NTvar{B}] \label{eq:ldpda-pda-rules-2-nf-8} \\
    p, \nestedstack \ntvar{X} [r, \rest \NTvar{A}] &\xoutarrow{\varepsilon} q, \nestedstack \ntvar{Y} [q_\init, \NTvar{S}] \ntvar{Z} [s, \rest] \label{eq:ldpda-pda-rules-2-nf-9} \\
    % p, \nestedstack \ntvar{X} [r, \rest \NTvar{A}] &\xoutarrow{\varepsilon} q, \nestedstack \ntvar{Y} [s, \rest \NTvar{B} \NTvar{C}] \label{eq:ldpda-pda-rules-2-nf-10} \\
    % p, \nestedstack \ntvar{X} [r, \rest \NTvar{A}] &\xoutarrow{\varepsilon} q, \nestedstack \ntvar{Y} [s, \rest \NTvar{B}] \label{eq:ldpda-pda-rules-2-nf-11} \\
    p, \nestedstack \ntvar{X} [r, \rest \NTvar{A}] &\xoutarrow{\varepsilon} q, \nestedstack \ntvar{Y} [s, \rest]  \label{eq:ldpda-pda-rules-2-nf-12}\\
    p, \nestedstack \ntvar{X} [r, \NTvar{A}] &\xoutarrow{\symvar{a}} q, \nestedstack \label{eq:ldpda-pda-rules-2-nf-13}
\end{align}
\caption{Rules of PDA $\control$ PDA in normal form.}
\label{fig:ldpda-pda-rules-2-nf}
\end{figure}
% \david{The last rule in \cref{fig:ldpda-pda-rules-2-nf} used to have a slash in it -- did I edit it correctly?}

\cref{fig:ldpda-pda-derivation} shows a run of a PDA $\control$ PDA.
\begin{figure}
    \centering
    \footnotesize
    \begin{align*}
        (p, \nt{S_1} [q, \NT{S_2}], abab) 
        &\Rightarrow (p, \nt{S_1} [q, \NT{L_5} \NT{T}], abab) \\
        &\Rightarrow (p, \nt{S_1} [q, \NT{L_5} \NT{L_3} \NT{L_6}], abab) \\
        &\Rightarrow (p, \nt{S_1} [q, \NT{L_5} \NT{L_3} \NT{T} \NT{L_1}], abab) \\
        &\Rightarrow (p, \nt{S_1} [q, \NT{T} \NT{L_3} \NT{L_5}] \nt{A}[q, \NT{S_2}], abab) \\
        % &\Rightarrow (p, \nt{S_1} [q, \NT{T} \NT{L_3} \NT{L_5}] \nt{A}[q, \NT{L_5} \NT{T}], abab) \\
        % &\Rightarrow (p, \nt{S_1} [q, \NT{T} \NT{L_3} \NT{L_5}] \nt{A}[q, \NT{L_5}], abab) \\
        &\Rightarrow^3 (p, \nt{S_1} [q, \NT{L_5} \NT{L_3} \NT{T}], bab) \\
        &\Rightarrow (p, \nt{S_1} [q, \NT{L_5} \NT{L_3} \NT{L_4} \NT{L_7}], bab) \\
        &\Rightarrow (p, \nt{S_1} [q, \NT{L_5} \NT{L_3} \NT{L_4} \NT{T} \NT{L_2}], bab) \\
        &\Rightarrow (p, \nt{S_1} [q, \NT{L_5} \NT{L_3} \NT{L_4} \NT{T}] \nt{B} [q, \NT{S_2}] , bab) \\
        % &\Rightarrow (p, \nt{S_1} [q, \NT{L_5} \NT{L_3} \NT{L_4} \NT{T}] \nt{B} [q, \NT{L_5 T}] , bab) \\
        % &\Rightarrow (p, \nt{S_1} [q, \NT{L_5} \NT{L_3} \NT{L_4} \NT{T}] \nt{B} [q, \NT{L_5}] , bab) \\
        &\Rightarrow^3 (p, \nt{S_1} [q, \NT{L_5} \NT{L_3} \NT{L_4} \NT{T}], ab) \\
        &\Rightarrow (p, \nt{S_1} [q, \NT{L_5} \NT{L_3} \NT{L_4}], ab) \\
        &\Rightarrow (p, \nt{B} [q, \NT{S_2}] \nt{S_1} [q, \NT{L_5} \NT{L_3}], ab) \\
        &\Rightarrow (p, \nt{B} [q, \NT{S_2}] \nt{S_1} [q, \NT{L_5}] \nt{A} [q, \NT{S_2}], ab) \\
        % &\Rightarrow (p, \nt{B} [q, \NT{S_2}] \nt{S_1} [q, \NT{L_5}] \nt{A} [q, \NT{L_5 T}], ab) \\
        % &\Rightarrow (p, \nt{B} [q, \NT{S_2}] \nt{S_1} [q, \NT{L_5}] \nt{A} [q, \NT{L_5}], ab) \\
        &\Rightarrow^3 (p, \nt{B} [q, \NT{S_2}] \nt{S_1} [q, \NT{L_5}], b) \\
        &\Rightarrow (p, \nt{B} [q, \NT{S_2}], b) \\
        % &\Rightarrow (p, \nt{B} [q, \NT{L_5 T}], b) \\
        % &\Rightarrow (p, \nt{B} [q, \NT{L_5}], b) \\
        &\Rightarrow^3 (p, \varepsilon, \varepsilon)
    \end{align*}
    \caption{Example of a run in a PDA $\control$ PDA. 
    % The LD-PDA's configurations are augumented with the substring left to scan.
    }
    \label{fig:ldpda-pda-derivation}
\end{figure}

\begin{defin}
A run of a LD-PDA $\pushdown_1$ controlled by a PDA $\pushdown_2$ is \defn{accepting} if its initial configuration is $(q_\init, \ntvar{S}[q'_\init, \NTvar{S}]$, where $(q_\init,\ntvar{S})$ and $(q'_\init,\NTvar{S})$ are the initial configurations of $\pushdown_1$ and $\pushdown_2$, and its final configuration is $(q_\final,\varepsilon)$, where $(q_\final,\varepsilon)$ is $\pushdown_1$'s final configuration. 
\end{defin}

\begin{defin}
The \defn{language} recognized by an LD-PDA controlled by a PDA is the set of strings scanned by all the accepting paths.
\end{defin}

\begin{proposition}
An LD-PDA controlled by a PDA is \topeqJJ{} to an EPDA.
\end{proposition}

% \begin{proof}
%     See \cref{app:d-strong-eq}
% \end{proof}



% \begin{figure}[!h]
% \footnotesize
% \begin{align}
%     p, \nestedstack \ntvar{X} [r, \rest \NTvar{A}] &\xrightarrow{\varepsilon} p, \nestedstack \ntvar{X} [s, \rest \NTvar{B} \NTvar{C}]  \\
%     p, \nestedstack \ntvar{X} [r, \rest \NTvar{A}] &\xoutarrow{a/\varepsilon} q, \nestedstack \ntvar{Y} [s, \rest \NTvar{B} \NTvar{C}] \ntvar{Z}[s, \NTvar{S}]  \\
%     p, \nestedstack \ntvar{X} [r, \rest \NTvar{A}] &\xoutarrow{a/\varepsilon} q, \nestedstack \ntvar{Y} [s, \rest \NTvar{B}] \ntvar{Z}[s, \NTvar{S}] \\
%     p, \nestedstack \ntvar{X} [r, \rest \NTvar{A}] &\xoutarrow{a/\varepsilon} q, \nestedstack \ntvar{Y} [s, \rest] \ntvar{Z}[s, \NTvar{S}] \\
%     p, \nestedstack \ntvar{X} [r, \rest \NTvar{A}] &\xoutarrow{a/\varepsilon} q, \nestedstack \ntvar{Y} [s, \NTvar{S}] \ntvar{Z} [s, \rest \NTvar{B} \NTvar{C}] \\
%     p, \nestedstack \ntvar{X} [r, \rest \NTvar{A}] &\xoutarrow{a/\varepsilon} q, \nestedstack \ntvar{Y} [s, \NTvar{S}] \ntvar{Z} [s, \rest \NTvar{B}] \\
%     p, \nestedstack \ntvar{X} [r, \rest \NTvar{A}] &\xoutarrow{a/\varepsilon} q, \nestedstack \ntvar{Y} [s, \NTvar{S}] \ntvar{Z} [s, \rest] \\
%     p, \nestedstack \ntvar{X} [r, \rest \NTvar{A}] &\xoutarrow{a} q, \nestedstack \ntvar{Y} [s, \rest \NTvar{B} \NTvar{C}] \\
%     p, \nestedstack \ntvar{X} [r, \rest \NTvar{A}] &\xoutarrow{a} q, \nestedstack \ntvar{Y} [s, \rest \NTvar{B}] \\
%     p, \nestedstack \ntvar{X} [r, \rest \NTvar{A}] &\xoutarrow{a} q, \nestedstack \ntvar{Y} [s, \rest] \\
%     p, \nestedstack \ntvar{X} [r, \NTvar{A}] &\xoutarrow{a} q, \nestedstack 
% \end{align}
% \caption{Production rules of an LD-PDA controlled by a PDA in CNF.}
% \label{fig:ldpda-pda-rules-cnf}
% \end{figure}

% \subsubsection{Equivalence with EPDA}

% \begin{theorem}
% The formal system defined by a LD-PDA controlled by a PDA is topologically equivalent to EPDA.
% \end{theorem}

% \begin{proof}
% Sketch:

% $(\Rightarrow)$ Let $\pushdown_1 = (\states_1, \alphabet_1, \stackalphabet_1, \trans_1, (q_{i,1}, \NTvar{S}_1), (q_{f,1}, \varepsilon))$ be a controller PDA and $\pushdown_2 = (\states_2, \alphabet_2, \alphabet_1, \stackalphabet_2, \trans_2, (q_{i,2}, \NTvar{S}_2), (q_{f,2}, \varepsilon))$ an LD-PDA. We assume that both PDAs are in normal form. We can construct the EPDA $\pushdown = (\states, \alphabet, \stackalphabet, \trans, (q_i, [[\NTvar{S}]]), (q_f, \varepsilon))$ where

% $(\Leftarrow)$ Let $\pushdown = (\states, \alphabet, \stackalphabet, \trans, (q_i, [[\NTvar{S}]]), (q_f, \varepsilon))$ be an EPDA in normal form. Construct the controller PDA $\pushdown_1 = (\states_1, \alphabet_1, \stackalphabet_1, \trans_1, (q_{i,1}, \NTvar{S}_1), (q_{f,1}, \varepsilon))$ where $\states_1 = \{p \}$, $\stackalphabet_1 = \stackalphabet$, $q_{i,1}=p$, $q_{f,1}=p$ and $\NTvar{S}_1 = \NTvar{S}$. The LD-PDA $\pushdown_2 = (\states_2, \alphabet_2, \alphabet_1, \stackalphabet_2, \trans_2, (q_{i,2}, \NTvar{S}_2), (q_{f,2}, \varepsilon))$ is such that $\states_2 = \states$, $\alphabet_2 = \alphabet$, $\stackalphabet = \{\ntvar{X} \}$, $q_{i,2} = q_i$ and $q_{f,2}=q_f$. For each transition $p, \nestedstack [\rest \NTvar{A} \xrightarrow{\symvar{a}} q, \nestedstack [\rest \stackseq$, $p, \nestedstack [\rest \NTvar{A} \xrightarrow{\symvar{a}} q, \nestedstack [\NTvar{S}] [\rest \stackseq$ or $p, \nestedstack [\rest \NTvar{A} \xrightarrow{\symvar{a}} q, \nestedstack [\rest \stackseq [\NTvar{S}$ in $\trans$, add a label $\ell$ to $\alphabet_1$, a transition $p, \ntvar{X} \xrightarrow{\symvar{a}} q, \dist{\ntvar{X}}$, $p, \ntvar{X} \xrightarrow{\symvar{a}} q, \ntvar{X} \dist{\ntvar{X}}$ or $p, \ntvar{X} \xrightarrow{\symvar{a}} q, \dist{\ntvar{X}} \ntvar{X}$, respectively, to $\trans_2$ and a transition $p, \NTvar{A} \xrightarrow{\ell} p, \stackseq$ to $\trans_1$.
% \end{proof}


\subsection{CFG $\control$ PDA}

The LD-PDA's transitions and the controller CFG's productions can be merged by augmenting the PDA's stack symbols with sentential forms of the controller. The transitions in an LD-PDA controlled by a CFG can either change the sentential form of the top stack symbol (\cref{fig:ldpda-cfg-rules-2-nf}, \crefrange{eq:ldpda-cfg-rules-2-nf-1}{eq:ldpda-cfg-rules-2-nf-4}), or remove a terminal symbol $\ell$ from the top stack symbol's sentential form and apply a production labeled with $\ell$ of the LD-PDA (\cref{fig:ldpda-cfg-rules-2-nf}, \crefrange{eq:ldpda-cfg-rules-2-nf-5}{eq:ldpda-cfg-rules-2-nf-8}). The remaining sentential form is passed to the distinuished stack symbol of the right-hand side of $\ell$ and every other stack symbols gets augmented with the controller's start symbol. 

\begin{figure}[!h]
\footnotesize
\begin{align}
p, \nestedstack \ntvar{X} [\NTvar{A} \rest] &\xrightarrow{\varepsilon} p, \nestedstack \ntvar{X} [\NTvar{B} \NTvar{C} \rest] \label{eq:ldpda-cfg-rules-2-nf-1} \\
p, \nestedstack \ntvar{X} [\NTvar{A} \rest] &\xrightarrow{\varepsilon} p, \nestedstack \ntvar{X} [\NTvar{B} \rest] \label{eq:ldpda-cfg-rules-2-nf-2} \\
p, \nestedstack \ntvar{X} [\NTvar{A} \rest] &\xrightarrow{\varepsilon} p, \nestedstack \ntvar{X} [ \rest] \label{eq:ldpda-cfg-rules-2-nf-3} \\
p, \nestedstack \ntvar{X} [\NTvar{A} \rest] &\xrightarrow{\varepsilon} p, \nestedstack \ntvar{X} [\ell \rest] \label{eq:ldpda-cfg-rules-2-nf-4} \\
p, \nestedstack \ntvar{X} [\ell \rest] &\xoutarrow{\varepsilon} q, \nestedstack \ntvar{Y} [ \rest] \ntvar{Z} [\NTvar{S}] \label{eq:ldpda-cfg-rules-2-nf-5} \\
p, \nestedstack \ntvar{X} [\ell \rest] &\xoutarrow{\varepsilon} q, \nestedstack \ntvar{Y} [\NTvar{S}] \ntvar{Z} [ \rest] \label{eq:ldpda-cfg-rules-2-nf-6} \\
p, \nestedstack \ntvar{X} [\ell \rest] &\xoutarrow{\varepsilon} q, \nestedstack \ntvar{Y} [ \rest] \label{eq:ldpda-cfg-rules-2-nf-7} \\
p, \nestedstack \ntvar{X} [\ell] &\xoutarrow{\symvar{a}} q, \nestedstack \label{eq:ldpda-cfg-rules-2-nf-8}
\end{align}
\caption{Rules of CFG $\control$ PDA in normal form.}
\label{fig:ldpda-cfg-rules-2-nf}
\end{figure}
% \david{the last rule of \cref{eq:ldpda-cfg-rules-2-nf-8} used to have a slash in it. did i edit it correctly?}

% We reuse notions such as configuration and run, defined in the context of PDAs. We can thus define an accepting run as follows.
\begin{defin}
A run in a LD-PDA $\pushdown$ controlled by a CFG $\grammar$ is \defn{accepting} if the initial configuration is $(q_\init,\ntvar{S}[\NTvar{S}])$, where $(q_\init,\ntvar{S})$ is $\pushdown$'s initial configuration and $\NTvar{S}$ is $\grammar$'s start symbol, and $(q_\final,\varepsilon)$ is the final configuration, where $(q_\final,\varepsilon)$ is $\pushdown$'s final configuration. The \defn{language} of $\pushdown$ controlled by a CFG $\grammar$ is the set of strings scanned by all the accepting paths.  
\end{defin}

\cref{fig:ldpda-cfg-derivation} shows a run in a CFG $\control$ PDA.

\begin{figure}
    \footnotesize
    \centering
    \begin{align*}
\firsteq{(p, \nt{S_1}[\NT{S_2}], \sym{abbabb})} \\
&\Rightarrow (p, \nt{S_1}[\NT{T}\Sym{\ell_5}], \sym{abbabb}) \\
&\Rightarrow (p, \nt{S_1}[\Sym{\ell_1}\NT{T}\Sym{\ell_3}\Sym{\ell_5}], \sym{abbabb}) \\
&\Rightarrow (p, \nt{A}[\NT{S_2}] \nt{S_1}[\NT{T}\Sym{\ell_3}\Sym{\ell_5}], \sym{abbabb}) \\
% &\Rightarrow (p, \nt{A}[\NT{T}\Sym{\ell}_5] \nt{S_1}[\NT{T}\Sym{\ell_3}\Sym{\ell_5}], \sym{abbabb}) \\
% &\Rightarrow (p, \nt{A}[\Sym{\ell}_5] \nt{S_1}[\NT{T}\Sym{\ell_3}\Sym{\ell_5}], \sym{abbabb}) \\
&\Rightarrow^3 (p, \nt{S_1}[\NT{T}\Sym{\ell_3}\Sym{\ell_5}], \sym{bbabb}) \\
&\Rightarrow (p, \nt{S_1}[\Sym{\ell_2}\NT{T}\Sym{\ell_4}\Sym{\ell_3}\Sym{\ell_5}], \sym{bbabb}) \\
&\Rightarrow (p, \nt{B}[\NT{S}_2] \nt{S_1}[\NT{T}\Sym{\ell_4}\Sym{\ell_3}\Sym{\ell_5}], \sym{bbabb}) \\
% &\Rightarrow (p, \nt{B}[\NT{T} \Sym{\ell}_5] \nt{S_1}[\NT{T}\Sym{\ell_4}\Sym{\ell_3}\Sym{\ell_5}], \sym{bbabb}) \\
% &\Rightarrow (p, \nt{B}[\Sym{\ell}_5] \nt{S_1}[\NT{T}\Sym{\ell_4}\Sym{\ell_3}\Sym{\ell_5}], \sym{bbabb}) \\
&\Rightarrow^3 (p, \nt{S_1}[\NT{T}\Sym{\ell_4}\Sym{\ell_4}\Sym{\ell_3}\Sym{\ell_5}], \sym{babb}) \\
&\Rightarrow (p, \nt{S_1}[\Sym{\ell_2}\NT{T}\Sym{\ell_4}\Sym{\ell_4}\Sym{\ell_3}\Sym{\ell_5}], \sym{babb}) \\
&\Rightarrow (p, \nt{B}[\NT{S}_2] \nt{S_1}[\NT{T}\Sym{\ell_4}\Sym{\ell_4}\Sym{\ell_3}\Sym{\ell_5}], \sym{babb}) \\
% &\Rightarrow (p, \nt{B}[\NT{T} \Sym{\ell}_5] \nt{S_1}[\NT{T}\Sym{\ell_4}\Sym{\ell_4}\Sym{\ell_3}\Sym{\ell_5}], \sym{babb}) \\
% &\Rightarrow (p, \nt{B}[\Sym{\ell}_5] \nt{S_1}[\NT{T}\Sym{\ell_4}\Sym{\ell_4}\Sym{\ell_3}\Sym{\ell_5}], \sym{babb}) \\
&\Rightarrow^3 (p, \nt{S_1}[\Sym{\ell_4}\Sym{\ell_4}\Sym{\ell_3}\Sym{\ell_5}], \sym{abb}) \\
&\Rightarrow (p, \nt{S_1}[\Sym{\ell_4}\Sym{\ell_3}\Sym{\ell_5}] \; \nt{B}[\NT{S_2}], \sym{abb}) \\
&\Rightarrow (p, \nt{S_1}[\Sym{\ell_3}\Sym{\ell_5}] \; \nt{B}[\NT{S_2}] \; \nt{B}[\NT{S_2}], \sym{abb}) \\
&\Rightarrow (p, \nt{S_1}[\Sym{\ell_5}] \; \nt{A}[\NT{S_2}] \; \nt{B}[\NT{S_2}] \; \nt{B}[\NT{S_2}], \sym{abb}) \\
&\Rightarrow (p, \nt{A}[\NT{S_2}] \; \nt{B}[\NT{S_2}] \; \nt{B}[\NT{S_2}], \sym{abb}) \\
% &\Rightarrow (p, \nt{A}[\NT{T}\Sym{\ell_5}] \; \nt{B}[\NT{S_2}] \; \nt{B}[\NT{S_2}], \sym{abb}) \\
% &\Rightarrow (p, \nt{A}[\Sym{\ell_5}] \; \nt{B}[\NT{S_2}] \; \nt{B}[\NT{S_2}], \sym{abb}) \\
&\Rightarrow^3 (p, \nt{B}[\NT{S_2}] \; \nt{B}[\NT{S_2}], \sym{bb}) \\
% &\Rightarrow (p, \nt{B}[\NT{T}\Sym{\ell_5}] \; \nt{B}[\NT{S_2}], \sym{bb}) \\
% &\Rightarrow (p, \nt{B}[\Sym{\ell_5}] \; \nt{B}[\NT{S_2}], \sym{bb}) \\
&\Rightarrow^3 (p, \nt{B}[\NT{S_2}], \sym{b}) \\
% &\Rightarrow (p, \nt{B}[\NT{T}\Sym{\ell_5}], \sym{b}) \\
% &\Rightarrow (p, \nt{B}[\Sym{\ell_5}], \sym{b}) \\
&\Rightarrow^3 (p, \varepsilon, \varepsilon).
\end{align*}
    \caption{Example of a run in a CFG $\control$ PDA. 
    % The PDA's configurations are augumented with the substring left to scan.
    }
    \label{fig:ldpda-cfg-derivation}
\end{figure}

% \begin{figure}[!h]
% \footnotesize
% \begin{align}
% p, \nestedstack \ntvar{X} [\NTvar{A} \rest] &\xrightarrow{\varepsilon} p, \nestedstack \ntvar{X} [\NTvar{B} \NTvar{C} \rest] \\
% p, \nestedstack \ntvar{X} [\NTvar{S} \rest] &\xrightarrow{\varepsilon} p, \nestedstack \ntvar{X} [ \rest] \\
% p, \nestedstack \ntvar{X} [\NTvar{A} \rest] &\xrightarrow{\varepsilon} p, \nestedstack \ntvar{X} [a \rest] \\
% p, \nestedstack \ntvar{X} [a \rest] &\xoutarrow{a/\varepsilon} , \nestedstack \ntvar{Y} [ \rest] \ntvar{Z} [\NTvar{S}] \\
% p, \nestedstack \ntvar{X} [a \rest] &\xoutarrow{a/\varepsilon} , \nestedstack \ntvar{Y} [\NTvar{S}] \ntvar{Z} [ \rest] \\
% p, \nestedstack \ntvar{X} [a \rest] &\xoutarrow{a} , \nestedstack \ntvar{Y} [ \rest] \\
% p, \nestedstack \ntvar{X} [a] &\xoutarrow{a} , \nestedstack \\
% p, \nestedstack \ntvar{S} [a] &\xoutarrow{\varepsilon} , \nestedstack
% \end{align}
% \caption{Production rules of an LD-PDA controlled by a CFG in CNF.}
% \label{fig:ldpda-cfg-rules-cnf}
% \end{figure}

% \begin{proof}
%     See \cref{app:d-strong-eq}
% \end{proof}

\begin{proposition}
CFG $\control$ CFG, PDA $\control$ CFG, CFG $\control$ PDA and PDA $\control$ PDA are \bijeqJJ{}.
\end{proposition}

% \begin{proof}
%     See \cref{app:d-weak-eq}.
% \end{proof}
